On subtrees of the representation tree in rational base numeration systems

Every rational number p/q defines a rational base numeration system in which every integer has a unique finite representation, up to leading zeroes. This work is a contribution to the study of the set of the representations of integers. This prefix-closed subset of the free monoid is naturally represented as a highly non-regular tree. Its nodes are the integers, its edges bear labels taken in {0,1,...,p-1}, and its subtrees are all distinct. We associate with each subtree (or with its root n) three infinite words. The bottom word of n is the lexicographically smallest word that is the label of a branch of the subtree. The top word of n is defined similarly. The span-word of n is the digitwise difference between the latter and the former. First, we show that the set of all the span-words is accepted by an infinite automaton whose underlying graph is essentially the same as the tree itself. Second, we study the function that computes for all n the bottom word associated with n+1 from the one associated with n, and show that it is realised by an infinite sequential transducer whose underlying graph is once again essentially the same as the tree itself. An infinite word may be interpreted as an expansion in base p/q after the radix point, hence evaluated to a real number. If T is a subtree whose root is n, then the evaluations of the labels of the branches of T form an interval of $\mathbb{R}$. The length of this interval is called the span of n and is equal to the evaluation of the span-word of n. The set of all spans is then a subset of R and we use the preceding construction to study its topological closure. We show that it is an interval when p is greater than or equal to 2q-1, and a Cantor set of measure zero otherwise.

==> extra_lemma.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{ Hausdorff dimension of span-sets in large bases~$(p>2\xmd q -1)$}
\lsection{Hau-dim-spa}

%
The notion of Hausdorff dimension is classical when studying fractals
(\cf~\cite{Falc14}).
%
Given a set~$F$, the \emph{$d$-dimensional Hausdorff measure} of~$F$ is defined by
\begin{equation*}
  \hausmeas[d]{F} = \lim_{\epsilon \rightarrow 0}~\inf \left\{~ \sum_i{} {r_i}^{\!d} ~~\middle|~~
    \begin{array}{@{}l}
    \text{there is a countable cover of }F\text{ by balls } B_0,B_1,\ldots\\
    \text{such that for every }i\text{, }B_i\text{ has radius }r_i\text{ and }r_i\mathbin{<}\epsilon.
    \end{array}
  \right\}\eqpnt
\end{equation*}
Then, the Hausdorff dimension of~$F$ is defined by:
\begin{equation*}
  \hausdim{F} = \inf\left\{ d\mathbin{\geq}0 ~\middle|~ \hausmeas{F} \mathbin{=} 0\right\} \eqpnt
\end{equation*}
%
It is known that the Hausdorff dimension of the Ternary Cantor set
is~$\frac{\ln(2)}{\ln(3)}$.
%
We conjecture that a similar statement holds for~$\adh{\Spq}$.
%


\begin{conjecture}\lconjecture{haus-dime}
  If~$p> 2q-1$, the Hausdorff dimension of~$\adh{\Spq}$ is equal to~$\frac{\ln(2q-1)}{\ln(p)}$.
\end{conjecture}

%
We give here the proof of half this conjecture.
%

%

\begin{proposition}\lproposition{haus}
  If~$p> 2q-1$,
  the Hausdorff dimension of~$\adh{\Spq}$ is smaller than or equal
  to~$\frac{\ln(2q-1)}{\ln(p)}$.
\end{proposition}

\begin{proof}
  Let~$r$ be a positive real number.
  %
  We denote by~$N(r)$ the minimal number of interval of length~$r$
  required to cover~$\adh{\Spq}$.
  %
  Let~$d$ be a positive real number.
  %
  The remainder of the proof consists in majoring~$N(r)\xmd r^{d}$.
  %

%   We write~$y=\sup(\Spq)$.
  %
  Let~$i$ be the integer defined as follows:
  \begin{gather}
    i = \bceil{ \frac{\ln \omegapq - \ln r}{\ln z} }      \lequation{haus-i}
%     \\
%     \lequation{haus-r}
%     z^{i-1} \leq  \frac{\omegapq}{r} < z^i
  \end{gather}
  %
  Note in particular that from \rlemma{l-Iu-appr}, it holds:
%   of length~$i-1$:
  \begin{equation} \lequation{haus-l-Ui}
    \forall u\in \pref{\Wpq} \quantvrg \wlen{u}=i\quantsp \ell(\Iu)< \omegapq z^{-i} < r \eqpnt
  \end{equation}
  %
  Note also that~$i$ tends to infinity when~$r$ tends to~$0$.
  %

  \medskip


  %
  We denote by~$n$ the number of words in~$\pref{\Wpq}$ that are of length~$i$; in particular~$n-1$
  is the maximal integer that a length-$i$ word may be evaluated to, hence:
  \begin{gather}
    n-1 \leq \val{(p-1)^i} = \frac{p-1}{p-q} (z^{i}-1 ) < z (z^{i}-1) \notag\\
    n < z^{i+1} \lequation{haud-n-zi} \eqpnt
  \end{gather}
  %
  We write~$n$ in base~$p$ as a word~$x_k \xmd x_{k-1}\cdots x_0$ (which belongs to~$\Aps$); in other words,
  \begin{equation}
    n = \sum_{m=0}^{k} x_m p^m
  \end{equation}
  By definition,~$k < \frac{\ln n}{\ln p} + 1$, hence applying \requation*{haud-n-zi} yields
  the following
  \begin{equation}    \lequation{haus-k-and-i}
    k < \frac{\ln{n}}{\ln{p}} + 1 < (i+1)\xmd \frac{\ln{z}}{\ln{p}} +1
  \end{equation}
  %



%   \begin{equation*}
%     n =   \underbrace{p^k +\cdots + p^k}_{d_k\text{ times}}
%         + \underbrace{p^{k-1} + \cdots + p^{k-1}}_{d_{k-1}\text{ times}}
%         + \cdots
%         + \underbrace{p+\cdots+p}_{d_1 \text{ times}}
%         + \underbrace{1+\cdots+1}_{d_0 \text{ times}}
%   \end{equation*}
  %
  \begin{claim}\lclaim{haus-claim-i}
    Let~$j$ be an integer and~$U$ be~$p^j$
    words of length~$i\geq j$.
    %
    If~$\val{U}$ is an integer interval of size~$p^j$ then
    at most~$(2q-1)^j$ words in~$U$ belong to~$\Bpqs$.
  \end{claim}
  \begin{proofwithbar}
    The suffixes of length~$i$ of the words in~$U$ are exactly the words of the set~${\Ap}^{\!j}$
    (\rlemma{tpq-suff-prec}).
    %
    Among these suffixes, exactly~$(2q-1)^j$ belong to~$\Bpqs$.
    %
    The claim follows.
  \end{proofwithbar}
  %

  %
  The words of length~$i$ in~$\pref{\Wpq}$ are evaluated to the integers from~$0$
  to~$n-1$.
  %
  We split this integer interval~$\set{0,...,n-1}$ into integer subintervals as follows:~$x_k$ subintervals of cardinal~$p^k$,~$c_{k-1}$ subintervals of cardinal~$p^{k-1}$,
  \ldots,~$x_1$ subintervals of cardinal~$p$,~$x_0$ subintervals of cardinal~$1$.
  %
  Applying \rclaim{haus-claim-i} on each of these subintervals yields
  that there are at most~$\alpha$ words (defined below) of length~$i$ in~$\pref{\Wpq}$
  that belong to~$\Bpqs$:
  \begin{equation}\lequation{haus-alpha}
    \alpha = \sum_{m=0}^{k} x_m (2q-1)^m < \frac{p-1}{2q-2} (2q-1)^{k+1}\eqpnt
  \end{equation}
  %
  For each such word~$u$, one interval of length~$r$ is enough to cover~$I_u$ (from \requation*{haus-l-Ui}), hence
  \begin{equation}\lequation{haus-Nr}
    N(r) < \alpha \eqpnt
  \end{equation}
  %
  We major~$N(r)$ using \requation*{haus-alpha}+\requation*{haus-Nr} and~$r$ using \requation*{haus-i}, yielding:
%   Using \requation*{haus-r}, , it follows that
  \begin{equation*}
    N(r) \xmd  r^d < \eta \xmd (2q-1)^{k+1} \xmd z^{-(i-1)\xmd d} \quad\quad \text{with}\quad \eta = \frac{p-1}{2q-2} {\omegapq}^{\!\!d}\eqpnt
  \end{equation*}
  %
  Finally, majoring~$k$ using \requation*{haus-k-and-i}, we obtain:
  \begin{equation*}
    N(r) \xmd r^d < \beta \xmd \xmd z^{\left(\textstyle(i+1)\left(\frac{\ln(2q-1)}{\ln{p}} - d\right)\right)}
    \quad\quad\text{with}\quad\beta = \frac{p-1}{2q-2}\xmd {\omegapq}^{\!\!d} \xmd (2q-1)^2 \xmd z^{2\xmd d} \eqpnt
  \end{equation*}
%   \begin{equation*}
%     N(r) \xmd r^d < \frac{p-1}{2q-2}\xmd \frac{(2q-1)^2}{z^{2\xmd d}} \xmd y^d \xmd e^{(i+1) \xmd \ln (z) \xmd f(d) }
%     \quad\quad\text{with}\quad f(d) = \frac{\ln(2q-1)}{\ln{p}} - d \eqpnt
%   \end{equation*}
  %
%   Finally, majoring~$i$ thanks to \requation*{haus-i} we obtain:
%   \begin{equation*}
%     N(r) \xmd r^d < \underbrace{\frac{p-1}{2q-2}\xmd \frac{(2q-1)^2}{z^{2\xmd d}} \xmd y^d \xmd e^{(\ln(y\xmd z^2)-\ln(r)) \xmd  f(d) }}_{F(r,d)}
%     \quad\quad\text{with}\quad f(d) = \frac{\ln(2q-1)}{\ln{p}} - d \eqpnt
%   \end{equation*}
%   %

  %
  Let us fix~$d$ such that~$d>\frac{\ln(2q-1)}{\ln{p}}$.
  %
  When~$r$ tends to~$0$,~$i$ tends to~$+\infty$ and then, previous equation implies that~$N(r) \xmd r^d$
  tends to~$0$.
  %
  Since for every real~$r$, we may cover~$\adh{\Spq}$ with~$N(r)$ intervals of length~$r$,
  it holds
  \begin{equation*}
    \hausmeas[d]{\adh{\Spq}} \leq \lim_{r\rightarrow 0} N(r) \xmd r^d = 0 \eqpnt
  \end{equation*}
  %

  %
 Then, the Hausdorff dimension of~$\adh{\Spq}$ is at most~$\frac{\ln(2q-1)}{\ln{p}}$.
  %
\end{proof}


